2FE: Two-Factor Encryption for Cloud Storage

Encrypted cloud storage services are steadily increasing in popularity, with many commercial solutions currently available. In such solutions, the cloud storage is trusted for data availability, but not for confidentiality. Additionally, the user's device is considered secure, and the user is expected to behave correctly. We argue that such assumptions are not met in reality: e.g., users routinely forget passwords and fail to make backups, and users' devices get stolen or become infected with malware. Therefore, we consider a more extensive threat model, where users' devices are susceptible to attacks and common human errors are possible. Given this model, we analyze 10 popular commercial services and show that none of them provides good confidentiality and data availability. Motivated by the lack of adequate solutions in the market, we design a novel scheme called Two-Factor Encryption (2FE) that draws inspiration from two-factor authentication and turns file encryption and decryption into an interactive process where two user devices, like a laptop and a smartphone, must interact. 2FE provides strong confidentiality and availability guarantees, as it withstands compromised cloud storage, one stolen or compromised user device at a time, and various human errors. 2FE achieves this by leveraging secret sharing with additional techniques such as oblivious pseudorandom functions and zero-knowledge proofs. We evaluate 2FE experimentally and show that its performance overhead is small. Finally, we explain how our approach can be adapted to other related use cases such as cryptocurrency wallets.

==> figure-construction.tex <==
\newcommand\psep{\noindent\rule{\textwidth}{0.4pt}}

\begin{figure}[h]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\mathsf{2FE}[\kappa,G,q,H, H_{G},H_{b},\mathbf{AE},\mathbf{KDF},\mathbf{MAC}]$
    \end{center}
    The protocol is parameterized by a security parameter $\kappa$, cyclic group
    $G$ of order $q$ and hash functions $H:\bits^{*}\rightarrow\bits^{*}$, $H_{G}:\bits^{*}\rightarrow G$ and
    $H_{b}:\bits^{*}\times G\rightarrow\bits^{2\kappa}$; as well as an
    authenticated encryption scheme $\mathbf{AE}=(\Enc,\Dec)$, key derivation
    function $\mathbf{KDF}=\KDF$ and message authentication scheme
    $\mathbf{MAC}=(\Mac, \Ver)$.

    \psep
    
    \ppara{Init$^{\star}$.} $C$ picks values $k$, $k_{C}$, $\alpha_{C}$ and
    $\beta_{D}$ at random from $\set{1,\dots,q-1}$. Compute
    $k_{D}=k-k_{C}\mod{q}$, $\alpha_{S}=k_{D}-\alpha_{C}\mod{q}$ and
    $\beta_{S}=k_{C}-\beta_{D}\mod{q}$. (If any of these are 0, the sub-protocol
    is re-run.) Finally, send $(k_{D},\beta_{D})$ to $D$,
    $(\alpha_{S},\beta_{S})$ to $S$; record $(k_{C},\alpha_{C})$ and delete
    $(k,k_{D},\alpha_{S},\beta_{S},\beta_{D})$.

    \ppara{Encrypt.} Let $(pw,\mtag,m)$ be the input to $C$ and $\mtag$ the
    input to $D$. Run the following protocol:
    \begin{enumerate}
    \item $C$ pick at random $s\pick\bits^{k}$ and send $a=H_{G}(s)$ to $D$,
    \item $D$ compute $b=(\mtag\cdot a)^{k_{D}}$ and return $b$ to $C$,
    \item $C$ compute an encryption and authentication key as
      \[
        k_{\textsc{enc}} \concat k_{\textsc{mac}} = H_{b}(s,(\mtag\cdot a)^{k_{C}}\cdot b)=H_{b}(s,(\mtag\cdot H_{G}(s))^{k}).
      \]
    \end{enumerate}
    Compute the encryption of $m$ as $c=(\mtag, r, c_{s}, c_{m})$ where
    $c_{s}=\KDF(pw;r)\oplus s$ and $c_{m}=\Enc(k_{\textsc{enc}},m)$; compute
    $\sigma=\Mac(k_{\textsc{mac}},c)$ and upload $(\sigma,c)$ to $S$.

    % \ppara{TagCheck.} On input $\mtag$ to $C$: First send $\mtag$ to $S$. If $S$
    % has a record with tag $\mtag$, hand $\mtag$ to $D$, otherwise send $\bot$ to
    % $D$ who will then abort. If $D$ received a tag $\mtag'$ from $S$, show this
    % to $U$ and wait for a reply $\mathsf{rep}$. If $\mathsf{rep}=\mathtt{OK}$,
    % send $\mathtt{OK}$ to $S$; otherwise abort. If $S$ got an $\mathtt{OK}$ from
    % $D$, return the ciphertext pair $(\sigma, c)$ associated with $\mtag$ to $C$.

    \ppara{Decrypt.} Let $\mtag$ be the input to $C$, and $(pw,\mtag)$ the input
    to $C$. Obtain $(\sigma,c)$ from $S$, where $c=(\mtag,r,c_{s},c_{m})$ and
    compute $s=\KDF(pw;r)\oplus c_{s}$. $k_{\textsc{enc}}$ and
    $k_{\textsc{mac}}$ is then derived as above: $a=H_{G}(s)$ is sent to $D$,
    who replies with $b=(\mtag\cdot a)^{k_{C}}$, from which $C$ computes
    $k_{\textsc{enc}} \concat k_{\textsc{mac}} =H_{b}(s,(\mtag\cdot
    H_{G}(s))^{k})$.  If $\Ver(k_{\textsc{mac}},\sigma)=1$, output
    $\Dec(k_{\textsc{enc}},c_{m})$. Otherwise output $\bot$.

    \ppara{Refresh.} $C$ picks at random $z\pick\Z_{m}$, sets
    $k_{C}\leftarrow k_{C}+z$ and sends $z$ to $D$ and $S$. $D$ likewise sets
    $k_{D}\leftarrow k_{D}-z$, and $S$ sets $\alpha_{S}\leftarrow\alpha_{S}+z$
    and $\beta\leftarrow\beta_{S}-z$.
    
  \end{framed}
  \caption{asd}
  \label{fig:asd}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figure-construction2.tex <==
\begin{figure}[p]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\textsf{2FE}[G,p,H_{G},H_{b},\mathsf{AE},\mathsf{MAC},\mathsf{KDF},\mathsf{RF},\Ptwoprf,\mathsf{TG}]$
    \end{center}

    $G$ is a group of order $p$, $H_{G}$, $H_{b}$ are hash functions,
    $\mathsf{AE}=(\Enc,\Dec)$ is an authenticated encryption scheme,
    $\mathsf{MAC}=(\Mac,\Ver)$ a message authentication scheme and $\KDF$ a
    password based key derivation function. $\mathsf{RF}$ is the protocol
    defined in Figure~\ref{fig:refresh} and $\Ptwoprf$ is defined in
    Figure~\ref{fig:2pc-prf}. $\mathsf{TG}$ is a protocol for computing a file
    tags. Let $pw$ be the user's password.
    
    \ppara{Init.} $C$ picks $\keyC,\keyD,\alpha_{S},\beta_{S}\pick\Z_{q}$ and
    computes $\alpha_{C}=\keyD - \alpha_{S}$ and $\beta_{D}=\keyC - \beta_{S}$.
    Give $(\keyD,\beta_{D})$ to $D$, $(\alpha_{S},\beta_{S})$ to $S$ and store
    $(\keyC, \alpha_{C})$. Securely erase
    $\beta_{D},\beta_{S},\alpha_{S},\keyD$.
    
    \ppara{Encrypt.} With input $(pw, m)$ from $U$. On $C$
    \begin{enumerate}
    \item Pick $s\pick\bits^{\kappa}$ and run $\mathsf{TG}$ to generate a tag
      $t$.
    \item Send $(s,t)$ to $D$.
    \end{enumerate}
    $C$ and $D$ run \Ptwoprf\ where $C$ inputs $(t,s,\keyC)$ and $D$ inputs
    $(t,s,\keyD)$. Denote by $k_{\textsc{enc}}, k_{\textsc{mac}}$ the
    result. $C$ computes:
    \begin{enumerate}
    \item $c=(t,r,c_{s},c_{m})$ where $c_{s}=s\oplus\KDF(pw;r)$ and
      $c_{m}=\Enc(k_{\textsc{enc}},m)$.
    \item $\sigma=\Mac(k_{\textsc{mac}},c)$.
    \end{enumerate}
    Finally, $C$ uploads $\mathsf{ctxt}_{t}=(\sigma,c)$ to $S$.

    \ppara{Decrypt.} With input $(pw, t)$ from $U$.
    \begin{enumerate}
    \item $C$ sends $t$ to $S$, who checks if a record $\mathsf{ctxt}_{t}$ is
      stored. If not, $S$ returns $\bot$ to $C$. Otherwise, $S$ forwards
      $(t,r,c_{s})$ to $D$.
    \item $D$, on receiving $(t,r,c_{s})$ from $S$, shows $t$ to $U$. If $U$
      accepts (i.e., this $t$ matches the one $U$ input on $C$), then $U$ enters
      their password.
    \item $D$, if it received an accept from $U$, sends \texttt{OK} to $S$, who
      in turn sends $\mathsf{ctxt}_{t}$ to $C$.
    \end{enumerate}
    Both $C$ and $D$ can now recover $s$ as $s=\KDF(pw;r)$, after which
    \Ptwoprf\ is run to re-compute the appropriate encryption key. Having so
    obtained $k_{\textsc{enc}}$ and $k_{\textsc{mac}}$, $C$ first checks that
    $\Ver(k_{\textsc{mac}},\sigma)=1$, and if so, outputs
    $\Dec(k_{\textsc{enc}},c_{m})$.
    
  \end{framed}
  \caption{Device aided encryption protocol with recovery and key refreshment}
  \label{fig:concrete}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figures/de-pecs-exp.tex <==
\begin{figure}[h]
  % \centering
  \begin{framed}
  \textbf{Experiment} $\indECS^{\adv,b}_{\Pi}(\kappa)$

  \rule{\textwidth}{0.1mm}

  \begin{description}
  \item [Init] Set $\mathcal{T}\leftarrow\emptyset$, $b\pick\bits$ and $\mathsf{cc}\leftarrow \bot$.
  \item [Corrupt]: On $\cmda{corrupt}{P}$ for $P\in\set{\C,\D,\S}$ and if $\mathsf{cc}=\bot$, set $\mathsf{cc}\leftarrow P$.
    From this point on, any action taken by $P$ is performed by $\adv$ instead.

  \item [Encrypt] On $\cmda{encrypt}{f}$ from $\adv$, run $\pi_{\mathsf{enc}}(f)$.

  \item [Decrypt] On $\cmda{decrypt}{t}$ from $\adv$ and if $t\notin\mathcal{T}$, run $\pi_{\mathsf{dec}}(t)$.

  \item [Challenge] On $\cmda{challenge}{f,t}$ from $\adv$ and if $\mathsf{cc}\neq\C$.
    Run $\pi_{\mathsf{enc}}(t,f_{b})$ and let $\ctxt_{f}=(t,s,c)$ denote the ciphertext that is sent to $\S$.
    If $b=1$, set $\ctxt_{f}\leftarrow (t,s,r)$ with $r\pick\bits^{|c|}$.
    Send $\ctxt_{f}$ to $\S$.

  \item [Refresh] On $\cmd{refresh}$ from $\adv$.
    First take control of the corrupt party (if any).
    Run $\RF$ and set $\mathsf{cc}\leftarrow\bot$.

  \item [Output] On $\cmda{output}{b'}$ from $\adv$, output $b=b'$ and halt.

  \end{description}
\end{framed}
\caption{Device-enhanced E2EECS security experiment.}
  \label{fig:depecs}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/existingProviders.tex <==
%{
%	\def\margin{7pt}
%	\setlength\extrarowheight{\margin}
%	\begin{table*}[!t]
%		\caption{Overview of existing \ecs systems and their design choices: key material generation and storage; available key loss recovery mechanisms.}
%		\label{tab:existing_solutions}
%		\centering
%		\footnotesize
%		\begin{tabularx}{\textwidth}{m{.18\textwidth}m{.45\textwidth}m{.40\textwidth}}
%			\toprule
%			& \textsc{Key Generation and Protection} & \textsc{Recovery Mechanisms} \\[\margin]
%			\midrule
%
%			Mega~\cite{mega-security} & 
%			Key seeded from \underline{password}; \newline not stored on cloud & 
%			-- Recovery keys to download\\[\margin]
%
%			pCloud~\cite{pcloud-encrypted-cloud-storage} & 
%			Key seeded from \underline{password}; \newline not stored on cloud & 
%			\textit{(Not Possible)}\\[\margin]
%
%			Sync~\cite{sync-your-privacy} & 
%			Random master key; \newline stored encrypted w/ \underline{password} & 
%			-- Key memorized by client \newline -- Password hint on cloud \\[\margin]
%
%			SpiderOak~\cite{spideroak-no-knowledge} & 
%			Random key per file; \newline stored encrypted with the \underline{password} & 
%			-- Password hint on cloud \newline -- Key memorized by client \\[\margin]
%
%			Tresorit~\cite{tresorit-security} & 
%			Random key per file; \newline stored encrypted with the \underline{password} & 
%			-- Password in open client sessions \\[\margin]
%
%			Tarsnap~\cite{tarsnap} & 
%			Random master key; \newline not stored on cloud & 
%			\textit{(Not possible)}\\[\margin]
%			\bottomrule
%		\end{tabularx}
%	\end{table*}
%}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/exp-2pc-prf.tex <==
\begin{figure}[h]
\begin{framed}
  \textbf{Experiment} $\sfbf{Exp}^{\mathsf{kIND},c}_{\adv}(\kappa)$

  \textbf{Setup.} Let $B\leftarrow\emptyset$, $k\pick\Z_{q}$, and
  $t^{*}\leftarrow \mathsf{nil}$.

  \textbf{Query.} On input $\cmda{gen}{(t_{i},s_{i})}$ from $\adv$. If
  $t_{i}=t^{*}$ or $(t_{i},\cdot,\cdot,\cdot)\in B$, return $b$ and
  halt. Otherwise compute
  \begin{align*}
    a_{i}\leftarrow H_{1}(t_{i},s_{i}),
    && b_{i}\leftarrow a_{i}^{k},
    && \pi_{i}\pick\nizkDDH.\mathsf{Gen}(a_{i},b_{i},g^{k},k),
  \end{align*}
  and $B\leftarrow B\cup\set{(t_{i},s_{i},b_{i},\pi_{i})}$. Return $B$.

  \textbf{Challenge.}  On input $\cmda{challenge}{t}$ from $\adv$. If
  $t^{*}\neq\mathsf{nil}$, return. Otherwise, If $c=0$, pick
  $s\pick\bits^{\kappa}$ and define $Z\leftarrow (H_{1}(t,s))^{k}$. Otherwise,
  let $Z\pick G$ and compute a passing $\pi$ by programming $H$ accordingly. Set
  $t^{*}\leftarrow t$ and return $(t,s,Z,\pi)$.

  \textbf{Output}. On input $\cmda{output}{c'}$ by $\adv$, output
  $c'\stackrel{\tiny{?}}{=}c$ and halt.
\end{framed}
\caption{Key indistinguishability experiment. Note that the application of
  $H_{2}$ is local and so we ignore it here. Programming $H$ for the sake of
  creating a $\pi$ that passes is trivial, as the oracle picks the randomness.}
\label{fig:exp-kind}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/fulloverview.tex <==

\begin{figure}[tbp]
	\centering
	\subfloat[Intialization of keys.] {
		\scalebox{0.73}{
			\input{figures/overview_init.tex}
		}
	}\\
	\subfloat[Encryption of a file.] {
		\scalebox{0.73}{
			\input{figures/overview_enc.tex}
		}
	}\\
	\subfloat[Decryption of a file. User approval is requested only if policies specify so.] {
		\scalebox{0.73}{
			\input{figures/overview_dec.tex}
		}
	}\\
	\subfloat[Key recovery initiated by the client. The device is unavailable (e.g., loss) or cannot securely authenticate to the \name server.] {
		\scalebox{0.73}{
			\input{figures/overview_recovery.tex}
		}
	}
	\caption{High-level overview of the principal operations of \name. All operations are implicitly started by the user.}
	\label{fig:overview}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/intecs-exp.tex <==
\begin{figure}[h]
\begin{framed}
  \textbf{Experiment} $\intECS_{\Pi}^{\adv}(\kappa)$

  \rule{\textwidth}{0.1mm}
  
  \begin{description}
  \item [Init] Set $\mathsf{win}\leftarrow 0$, $\mathcal{V}\leftarrow\emptyset$ and $\mathsf{cc}\leftarrow\bot$.

  \item [Corruption] As in $\indECS$.
  \item [Refresh] As in $\indECS$.

  \item [Encrypt] On $\cmda{encrypt}{f}$ from $\adv$, run $\pi_{\mathsf{enc}}(f)$.
    Let $\ctxt_{f}$ be the result and set $\mathcal{V}\leftarrow\mathcal{V}\cup\set{\ctxt_{f}}$.

  \item [Decrypt] On $\cmda{decrypt}{f}$ from $\adv$.
    Run decryption $m\leftarrow\pi_{\mathsf{dec}}(t)$.
    If $\C$ is honest, $\ctxt_{f}\not\in\mathcal{V}$ and $m\neq\bot$ set $\mathsf{win}\leftarrow 1$.
    Output $m$.

  \item [Challenge] Behave as \emph{Decrypt} where $\C$ is honest.
    
  \item [Output] Output $\mathsf{win}$ and halt.
  \end{description}
\end{framed}
\caption{Integrity security experiment.}
  \label{fig:intecs}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> protocol-key-recovery.tex <==
\begin{figure}[h]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\RC[q]$
    \end{center}

    Suppose we wish to recover a client (the device case is symmetric).

    \begin{enumerate}
    \item \D\ sends \Cshare{D} to \C, and \S\ sends \Cshare{S} to \C.
    \item \C\ computes $\keyC = \Cshare{D} + \Cshare{S}$.
    \end{enumerate}

  \end{framed}
  \caption{Key refreshment protocol.}
  \label{fig:refresh}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> protocol-key-refresh.tex <==
\begin{figure}[h]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\mathsf{RF}[q]$
    \end{center}

    \begin{itemize}

    \item \C\ picks $z,\Cshare{C}\pick\Z_{q}$ and computes $\keyC\leftarrow \keyC + z$, and $\Cshare{S}=\keyC-\Cshare{C}$.
      Send \Cshare{S} to \S, and $z$ to \D.

    \item \D, on receiving $z$, computes $\keyD\leftarrow\keyD - z$.
      Pick $\Dshare{D}\pick\Z_{q}$, compute $\Dshare{S}=\keyD - \Dshare{D}$ and send \Dshare{S} to \S.
    \end{itemize}

  \end{framed}
  \caption{Key refreshment protocol.}
  \label{fig:refresh}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> protocol-steps.tex <==
Here is the list of protocol steps: 



==> protocol-tfe.tex <==
\begin{figure}[p]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\TFE[\kappa,G,p,H_{G},H_{b},\MAC,\AE,\KDF,\RF,\TG,\TPPRF]$
    \end{center}

    $G$ is a group of order $p$, $H_{G}$, $H_{b}$ are hash functions,
    $\mathsf{AE}=(\Enc,\Dec)$ is an authenticated encryption scheme,
    $\mathsf{MAC}=(\Mac,\Ver)$ a message authentication scheme and $\KDF$ a
    password based key derivation function. $\mathsf{RF}$ is the protocol
    defined in Figure~\ref{fig:refresh} and $\Ptwoprf$ is defined in
    Figure~\ref{fig:2pc-prf}. $\mathsf{TG}$ is a protocol for computing a file
    tags. Let $pw$ be the user's password. $\kappa$ is a security parameter.
    
    \ppara{Init.} $C$ picks $\keyC,\keyD,\alpha_{S},\beta_{S}\pick\Z_{q}$ and
    computes $\alpha_{C}=\keyD - \alpha_{S}$ and $\beta_{D}=\keyC - \beta_{S}$.
    Give $(\keyD,\beta_{D})$ to $D$, $(\alpha_{S},\beta_{S})$ to $S$ and store
    $(\keyC, \alpha_{C})$. Securely erase
    $\beta_{D},\beta_{S},\alpha_{S},\keyD$.
    
    \ppara{Encrypt.} With input $(pw, m)$ from $U$. On $C$
    \begin{enumerate}
    \item Pick $s\pick\bits^{\kappa}$ and run $\mathsf{TG}$ to generate a tag
      $t$.
    \item Send $(s,t)$ to $D$.
    \end{enumerate}
    $C$ and $D$ run \Ptwoprf\ where $C$ inputs $(t,s,\keyC)$ and $D$ inputs
    $(t,s,\keyD)$. Denote by $k_{\textsc{enc}}, k_{\textsc{mac}}$ the
    result. $C$ computes:
    \begin{enumerate}
    \item $c=(t,r,c_{s},c_{m})$ where $c_{s}=s\oplus\KDF(pw;r)$ and
      $c_{m}=\Enc(k_{\textsc{enc}},m)$.
    \item $\sigma=\Mac(k_{\textsc{mac}},c)$.
    \end{enumerate}
    Finally, $C$ uploads $\mathsf{ctxt}_{t}=(\sigma,c)$ to $S$.

    \ppara{Decrypt.} With input $(pw, t)$ from $U$.
    \begin{enumerate}
    \item $C$ sends $t$ to $S$, who checks if a record $\mathsf{ctxt}_{t}$ is
      stored. If not, $S$ returns $\bot$ to $C$. Otherwise, $S$ forwards
      $(t,r,c_{s})$ to $D$.
    \item $D$, on receiving $(t,r,c_{s})$ from $S$, shows $t$ to $U$. If $U$
      accepts (i.e., this $t$ matches the one $U$ input on $C$), then $U$ enters
      their password.
    \item $D$, if it received an accept from $U$, sends \texttt{OK} to $S$, who
      in turn sends $\mathsf{ctxt}_{t}$ to $C$.
    \end{enumerate}
    Both $C$ and $D$ can now recover $s$ as $s=\KDF(pw;r)\oplus c_{s}$, after which
    \Ptwoprf\ is run to re-compute the appropriate encryption key. Having so
    obtained $k_{\textsc{enc}}$ and $k_{\textsc{mac}}$, $C$ first checks that
    $\Ver(k_{\textsc{mac}},\sigma)=1$, and if so, outputs
    $\Dec(k_{\textsc{enc}},c_{m})$.
    
  \end{framed}
  \caption{Device aided encryption protocol with recovery and key refreshment}
  \label{fig:concrete}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> protocol-twopc-prf.tex <==
\begin{figure}[h]
  \begin{framed}
    \begin{center}
      \textbf{Protocol} $\TPPRF[G,p,H_{G},H_{b}]$
    \end{center}
    The protocol parameterized by a cyclic group $G$ of order $p$, hash functions
    $H_{b}:\bits^{*}\times G\rightarrow\bits^{*}$ and $H_{G}:\bits^{*}\rightarrow G$.
    \C\ has as input \keyC, $s$ and $t$; \D\ has as input \keyD, $s$ and $t$.
    \begin{description}

    \item[Send.] \D\ computes $b=(t\cdot H_{G}(s))^{\keyD}$ and sends $b$ to \C.

    \item[Compute] \C\ outputs
      $H_{b}(s,(t\cdot H_{G}(s))^{\keyC}\cdot b)=H_{b}(s,(t\cdot H_{G}(s))^{\PRFkey})$.

    \end{description}
  \end{framed}
  \caption{A two-party PRF protocol.}
  \label{fig:2pc-prf}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tikz-key-recovery.tex <==
\begin{figure}[h]

  \begin{framed}
    \textbf{Protocol} $\RC[q]$

    \centering
    
    \vspace{1em}

    \begin{tikzpicture}
      \node [box] (client) {
        \lbox{$\C$} {
          $\keyC\leftarrow \Cshare{D} + \Cshare{S}$
        }
      };
      \node [small box nc, right=3cm of client] (device) {\lbox{$\D$}{$\Cshare{D}$}};
      \node [small box nc, above right=1cm of client] (server) {\lbox{$\S$}{$\Cshare{S}$}};
      \draw [arrow] (server) -| node [above] {\arrowt{$\Cshare{S}$}} (client);
      \draw [arrow] (device) -- node [above] {\arrowt{$\Cshare{D}$}} (client);
    \end{tikzpicture}
  \end{framed}

  \caption{
    Client key recovery protocol (device key recovery is symmetric).
  }
  \label{fig:tikz-key-recovery}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tikz-nizk-ddh.tex <==
\begin{figure}[h]
  \centering
  \begin{framed}
    \textbf{Protocol} $\nizkDDH(g,y,a,b)$

    \vspace{1em}

    \begin{tikzpicture}
      \node [box] (device) {
        \lbox{$\D:g,a,b,y,\keyD$}{
          $t\pick\Z_{q}$ \\
          $w\leftarrow H_{3}(g,y,a,b,g^{t},a^{t})$
          $z\leftarrow t + w\cdot \keyD$
        }
      };
      \node [box, left=3cm of device] (client) {
        \lbox{$\C:g,a,b, y=g^{\keyD}$}{
          $\alpha\leftarrow g^{z}y^{-w}$, $\beta\leftarrow a^{z}b^{-w}$
          $w'\leftarrow H_{3}(g,y,a,b,\alpha,\beta)$
        }
      };
      \node [below=1.8em of client] (output) {};
      \draw [arrow] (device) -- node [above] {\arrowt{$\pi=(z,w)$}} (client);
      \draw [arrow] (client) -- node [right] {\arrowt{$w'\stackrel{?}{=}w$}} (output);
    \end{tikzpicture}
  \end{framed}
  \caption{Non-interactive proof in the Random Oracle model that something is a
    DDH tuple.}
  \label{fig:nizk-ddh}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tikz-tfe.tex <==
\begin{figure}[h]

  \begin{framed}
    \textbf{Protocol} $\TFE[\kappa,p,q,g,H_{g},H_{b},\MAC,\AE,\KDF,\TPPRF,\TG]$

    
    
    \vspace{1em}

    %% Encryption

    \textbf{Encryption:}

    \begin{center}
    
    \begin{tikzpicture}
      \node [small box] (user) {\lboxNR{\U}};
      \node [box, above=0.6cm of user] (client) {
        \lbox{$\C:\keyC$} {
          $r,s\pick\bits^{\kappa}$, $t\pick\TG$,
          $z=\TPPRF(s,t,\keyC)$,
          $\Kenc,\Kmac\leftarrow z$,
          $c_{s}\leftarrow\KDF(pw;r)$, $c_{m}\leftarrow\Enc(\Kenc,m)$,
          $c\leftarrow(t,r,c_{s},c_{m})$,
          $\sigma\leftarrow\Mac(\Kmac,c)$,
          $\ctxt\leftarrow(\sigma,c)$.
        }
      };
      \node [box, right=3cm of client] (device) {
        \lbox{$\D:\keyD$} {
          $\TPPRF(s,t,\keyD)$.
        }
      };
      \node [box, above right=1cm of client] (server) {
        \lbox{\S}{
          $\mathcal{D}\leftarrow\mathcal{D}\cup\set{\ctxt}$
        }
      };
      %
      \draw [arrow]
      (user)
      -- node [left] {\arrowt{$pw$, $m$}}
      node [right, pos=0.28] {\footnotesize{1}}
      (client);
      %
      \draw [arrow]
      (client.10)
      -- node [above] {\arrowt{$s$, $t$}}
      node [below, pos=0.05] {\footnotesize{2}}
      (device.170);
      %
      \draw [<->,shorten <=2pt, shorten >=2pt]
      (client.-15)
      -- node [above] {\arrowt{$\TPPRF$}}
      node [below, very near end] {\footnotesize{3}}
      (device.195);
      %
      \draw [arrow]
      (client)
      |- node [left] {\arrowt{\ctxt}}
      node [right, pos=0.1] {\footnotesize{4}}
      (server);
    \end{tikzpicture}
  \end{center}
  %% Decryption

  \textbf{Decryption:}
  \begin{center}
    \begin{tikzpicture}
      \node [box] (user) {
        \lbox{\U} {abort if $t\neq t'$}
      };
      \node [box, above=0.6cm of user] (client) {
        \lbox{$\C:\keyC$} {
          $s=\KDF(pw;r)\oplus c_{S}$.
          $z\leftarrow\TPPRF(s,t,\keyC)$
          $\Kenc,\Kmac\leftarrow z$,

          If $\Ver(\Kmac, \sigma) \neq 1$; $m\leftarrow\bot$.
          Else $m\leftarrow\Dec(\Kenc, c_{m})$.
        }
      };
      \node [box, right=3cm of client] (device) {
        \lbox{$\D:\keyD$} {
          Continue if \U\ sent \cmd{OK}.

          $s=\KDF(pw;r)\oplus c_{s}$,

          $\TPPRF(s,t,\keyD)$.
        }
      };
      \node [box, above right=1cm of client] (server) {
        \lbox{$\S:\mathcal{D}$}{
          If $(\sigma,(t',r,c_{s},c_{m}))\in\mathcal{D}$, continue.

          Continue if \C\ sent \cmd{OK}.
        }
      };
      %% User -- client
      \draw [arrow]
      (user.150)
      -- node [left] {\arrowt{$pw$, $t$}}
      node [right, pos=0.3] {\arrowt{1}}
      (client.-128);
      \draw [arrow]
      (client.-60)
      -- node [left] {\arrowt{$m$}}
      node [right, pos=0.3] {\arrowt{8}}
      (user.39);
      %%
      %% Client -- server
      %%
      \draw [arrow]
      (client.130)
      |- node [left] {\arrowt{$t'$}}
      node [right, pos=0.05] {\arrowt{2}}
      (server.165);
      \draw [arrow]
      (server.185)
      -| node [above, pos=0.3] {\arrowt{$(\sigma,(t',r,c_{s},c_{m}))$}}
      node [below, pos=0.05] {\arrowt{7}}
      (client.80);
      %%
      %% Server -- device
      %%
      \draw [arrow]
      (server)
      -| node [right] {\arrowt{$(t',r,c_{s})$}}
      node [above, pos=0.08] {\arrowt{3}}
      (device.50);
      \draw [arrow]
      (device.148)
      -- node [left] {\arrowt{$\bot$ or \cmd{OK}}}
      node [right, pos=0.15] {\arrowt{6}}
      (server.-50);
      %%
      %% user -- device
      %%
      \draw [arrow]
      (device.250)
      |- node [below] {\arrowt{$t'$}}
      node [left, pos=0.1] {\arrowt{4}}
      (user.10);
      \draw [arrow]
      (user.-10)
      -| node [below] {\arrowt{$\bot$ or $(\cmd{OK},pw)$}}
      node [above, pos=0.02] {\arrowt{5}}
      (device.-60);
      %%
      %% client -- device
      %%
      \draw [<->,shorten <=2pt, shorten >=2pt]
      (client)
      -- node [above] {\arrowt{$\TPPRF$}}
      node [below, pos=0.95] {\arrowt{6}}
      (device);
    \end{tikzpicture}
  \end{center}
  \end{framed}

  \caption{
    Device aided encryption protocol with recovery.
  }
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tikz-twopc-prf.tex <==
\begin{figure}[h]
  \begin{framed}

    \textbf{Protocol} $\TPPRF(t,s)$
    \centering
    \vspace{1em}

    \begin{tikzpicture}
      \node [box] (client) {
        \lbox{$\C:t,s,y,\keyC$}{
          $a\leftarrow (H_{1}(t\concat s))$ \\
          If $0=\nizkDDH(g,y,a,b)$ abort.
          \begin{align*}
            k&\leftarrow H_{2}(s,a\cdot b)\\
             &=H_{2}(s,(H_{1}(t\concat s))^{\PRFkey})
          \end{align*}
        }
      };
      \node [box, right=3cm of client] (device) {
        \lbox{$\D:t,s,\keyD$}{
          $b\leftarrow H_{1}(t\concat s)$, 
          $b\leftarrow a^{\keyD}$ \\
          $\pi\pick\nizkDDH(g,g^{\keyD},a,b)$
        }
      };
      \node [below=1.8em of client] (output) {};
      \draw [arrow] (device) -- node [above] {\arrowt{$b, \pi$}} (client);
      \draw [arrow] (client) -- node [right] {\arrowt{$k$}} (output);
    \end{tikzpicture}

  \end{framed}

  \caption{Two party PRF protocol. Where $\PRFkey=\keyC + \keyD$.}
  \label{fig:tikz-twoprf}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

